Model Stitching and Visualization How GAN Generators can Invert Networks in Real-Time

In this work, we propose a fast and accurate method to reconstruct activations of classification and semantic segmentation networks by stitching them with a GAN generator utilizing a 1x1 convolution. We test our approach on images of animals from the AFHQ wild dataset, ImageNet1K, and real-world digital pathology scans of stained tissue samples. Our results show comparable performance to established gradient descent methods but with a processing time that is two orders of magnitude faster, making this approach promising for practical applications.

==> eval_values/imagenetval_500/biggan.tex <==

--------------------------------------------------------------------
from layer: layer1, to layer: G.blocks.2.0
time taken: 7.50529146194458
mean cossim value: [tensor(0.8882)]
std cossim value: [tensor(0.0317)]
mean cossim gram matrices value: [tensor(0.9797)]
std cossim gram matrices value: [tensor(0.0132)]
mean value l1: [tensor(0.2543)]
std value l1: [tensor(0.0536)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer1, to layer: G.blocks.3.0
time taken: 7.553391456604004
mean cossim value: [tensor(0.9065)]
std cossim value: [tensor(0.0279)]
mean cossim gram matrices value: [tensor(0.9802)]
std cossim gram matrices value: [tensor(0.0141)]
mean value l1: [tensor(0.2302)]
std value l1: [tensor(0.0493)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer1, to layer: G.blocks.4.0
time taken: 7.81818151473999
mean cossim value: [tensor(0.8966)]
std cossim value: [tensor(0.0327)]
mean cossim gram matrices value: [tensor(0.9623)]
std cossim gram matrices value: [tensor(0.0257)]
mean value l1: [tensor(0.2416)]
std value l1: [tensor(0.0536)]
--------------------------------------------------------------------









from layer: layer2, to layer: G.blocks.2.0
time taken: 52.983317375183105
mean cossim value: [tensor(0.5555), tensor(0.8176), tensor(0.8195), tensor(0.8197), tensor(0.8198)]
std cossim value: [tensor(0.0409), tensor(0.0299), tensor(0.0298), tensor(0.0297), tensor(0.0297)]
mean cossim gram matrices value: [tensor(0.8410), tensor(0.9651), tensor(0.9659), tensor(0.9665), tensor(0.9659)]
std cossim gram matrices value: [tensor(0.0317), tensor(0.0166), tensor(0.0161), tensor(0.0161), tensor(0.0164)]
mean value l1: [tensor(0.2669), tensor(0.1632), tensor(0.1622), tensor(0.1620), tensor(0.1618)]
std value l1: [tensor(0.0263), tensor(0.0223), tensor(0.0223), tensor(0.0222), tensor(0.0222)]
--------------------------------------------------------------------
from layer: layer2, to layer: G.blocks.3.0
time taken: 6.546058893203735
mean cossim value: [tensor(0.8225)]
std cossim value: [tensor(0.0301)]
mean cossim gram matrices value: [tensor(0.9578)]
std cossim gram matrices value: [tensor(0.0211)]
mean value l1: [tensor(0.1600)]
std value l1: [tensor(0.0215)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer2, to layer: G.blocks.4.0
time taken: 6.662289381027222
mean cossim value: [tensor(0.7671)]
std cossim value: [tensor(0.0297)]
mean cossim gram matrices value: [tensor(0.9108)]
std cossim gram matrices value: [tensor(0.0274)]
mean value l1: [tensor(0.1853)]
std value l1: [tensor(0.0210)]
--------------------------------------------------------------------





--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.2.0
time taken: 8.38376784324646
mean cossim value: [tensor(0.6764)]
std cossim value: [tensor(0.0444)]
mean cossim gram matrices value: [tensor(0.8617)]
std cossim gram matrices value: [tensor(0.0394)]
mean value l1: [tensor(0.0985)]
std value l1: [tensor(0.0168)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.3.0
time taken: 5.519082307815552
mean cossim value: [tensor(0.5698)]
std cossim value: [tensor(0.0550)]
mean cossim gram matrices value: [tensor(0.7635)]
std cossim gram matrices value: [tensor(0.0625)]
mean value l1: [tensor(0.1142)]
std value l1: [tensor(0.0167)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.4.0
time taken: 5.7149975299835205
mean cossim value: [tensor(0.3973)]
std cossim value: [tensor(0.0573)]
mean cossim gram matrices value: [tensor(0.5817)]
std cossim gram matrices value: [tensor(0.0850)]
mean value l1: [tensor(0.1319)]
std value l1: [tensor(0.0140)]
--------------------------------------------------------------------







all models


--------------------------------------------------------------------
from layer: layer1, to layer: G.blocks.2.0
time taken: 23.489472150802612
model str: resnet34
mean cosine_similarity value: [tensor(0.7339), tensor(0.8883)]
std cosine_similarity value: [tensor(0.0404), tensor(0.0316)]
mean L1_Loss value: [tensor(0.4316), tensor(0.2541)]
std L1_Loss value: [tensor(0.0541), tensor(0.0534)]
mean cossim_gram_matrices value: [tensor(0.8739), tensor(0.9797)]
std cossim_gram_matrices value: [tensor(0.0384), tensor(0.0131)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.4657), tensor(0.6760)]
std cosine_similarity value: [tensor(0.0818), tensor(0.0919)]
mean L1_Loss value: [tensor(0.1187), tensor(0.0828)]
std L1_Loss value: [tensor(0.0181), tensor(0.0189)]
mean cossim_gram_matrices value: [tensor(0.6050), tensor(0.8671)]
std cossim_gram_matrices value: [tensor(0.1238), tensor(0.0813)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.6435), tensor(0.8558)]
std cosine_similarity value: [tensor(0.0481), tensor(0.0422)]
mean L1_Loss value: [tensor(0.1481), tensor(0.0790)]
std L1_Loss value: [tensor(0.0152), tensor(0.0149)]
mean cossim_gram_matrices value: [tensor(0.7168), tensor(0.9425)]
std cossim_gram_matrices value: [tensor(0.0768), tensor(0.0408)]
--------------------------------------------------------------------

--------------------------------------------------------------------
from layer: layer1, to layer: G.blocks.3.0
time taken: 23.88365340232849
model str: resnet34
mean cosine_similarity value: [tensor(0.7317), tensor(0.9066)]
std cosine_similarity value: [tensor(0.0405), tensor(0.0278)]
mean L1_Loss value: [tensor(0.4250), tensor(0.2300)]
std L1_Loss value: [tensor(0.0562), tensor(0.0493)]
mean cossim_gram_matrices value: [tensor(0.9016), tensor(0.9803)]
std cossim_gram_matrices value: [tensor(0.0367), tensor(0.0140)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.4734), tensor(0.6959)]
std cosine_similarity value: [tensor(0.0856), tensor(0.0876)]
mean L1_Loss value: [tensor(0.1144), tensor(0.0795)]
std L1_Loss value: [tensor(0.0174), tensor(0.0182)]
mean cossim_gram_matrices value: [tensor(0.6400), tensor(0.8617)]
std cossim_gram_matrices value: [tensor(0.1343), tensor(0.0876)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.6539), tensor(0.8727)]
std cosine_similarity value: [tensor(0.0544), tensor(0.0396)]
mean L1_Loss value: [tensor(0.1409), tensor(0.0734)]
std L1_Loss value: [tensor(0.0170), tensor(0.0144)]
mean cossim_gram_matrices value: [tensor(0.7616), tensor(0.9427)]
std cossim_gram_matrices value: [tensor(0.0827), tensor(0.0431)]
--------------------------------------------------------------------

from layer: layer1, to layer: G.blocks.3.0
time taken: 3.19014310836792
--------------------------------------------------------------------
--------------------------------------------------------------------
mean runtime: 3.1924480676651
std runtime: 0.08517392852009278



--------------------------------------------------------------------
from layer: layer1, to layer: G.blocks.4.0
time taken: 23.521106958389282
model str: resnet34
mean cosine_similarity value: [tensor(0.7185), tensor(0.8966)]
std cosine_similarity value: [tensor(0.0321), tensor(0.0327)]
mean L1_Loss value: [tensor(0.4509), tensor(0.2416)]
std L1_Loss value: [tensor(0.0464), tensor(0.0536)]
mean cossim_gram_matrices value: [tensor(0.8892), tensor(0.9623)]
std cossim_gram_matrices value: [tensor(0.0348), tensor(0.0257)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.4058), tensor(0.6920)]
std cosine_similarity value: [tensor(0.0636), tensor(0.0908)]
mean L1_Loss value: [tensor(0.1361), tensor(0.0806)]
std L1_Loss value: [tensor(0.0161), tensor(0.0183)]
mean cossim_gram_matrices value: [tensor(0.6609), tensor(0.8111)]
std cossim_gram_matrices value: [tensor(0.1179), tensor(0.1185)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.6426), tensor(0.8540)]
std cosine_similarity value: [tensor(0.0448), tensor(0.0485)]
mean L1_Loss value: [tensor(0.1416), tensor(0.0791)]
std L1_Loss value: [tensor(0.0137), tensor(0.0166)]
mean cossim_gram_matrices value: [tensor(0.7566), tensor(0.9151)]
std cossim_gram_matrices value: [tensor(0.0719), tensor(0.0617)]
--------------------------------------------------------------------




--------------------------------------------------------------------
from layer: layer2, to layer: G.blocks.2.0
time taken: 42.233357191085815
model str: resnet34
mean cosine_similarity value: [tensor(0.5606), tensor(0.8176), tensor(0.8193), tensor(0.8199), tensor(0.8198)]
std cosine_similarity value: [tensor(0.0413), tensor(0.0295), tensor(0.0294), tensor(0.0292), tensor(0.0297)]
mean L1_Loss value: [tensor(0.2636), tensor(0.1624), tensor(0.1614), tensor(0.1610), tensor(0.1608)]
std L1_Loss value: [tensor(0.0264), tensor(0.0218), tensor(0.0219), tensor(0.0218), tensor(0.0218)]
mean cossim_gram_matrices value: [tensor(0.8427), tensor(0.9660), tensor(0.9670), tensor(0.9676), tensor(0.9671)]
std cossim_gram_matrices value: [tensor(0.0331), tensor(0.0163), tensor(0.0155), tensor(0.0156), tensor(0.0165)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.3017), tensor(0.5913), tensor(0.5920), tensor(0.5924), tensor(0.5930)]
std cosine_similarity value: [tensor(0.0449), tensor(0.0547), tensor(0.0549), tensor(0.0547), tensor(0.0545)]
mean L1_Loss value: [tensor(0.0749), tensor(0.0541), tensor(0.0540), tensor(0.0538), tensor(0.0538)]
std L1_Loss value: [tensor(0.0067), tensor(0.0067), tensor(0.0067), tensor(0.0066), tensor(0.0066)]
mean cossim_gram_matrices value: [tensor(0.7070), tensor(0.9209), tensor(0.9182), tensor(0.9208), tensor(0.9201)]
std cossim_gram_matrices value: [tensor(0.0584), tensor(0.0326), tensor(0.0324), tensor(0.0323), tensor(0.0326)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4354), tensor(0.7732), tensor(0.7756), tensor(0.7762), tensor(0.7757)]
std cosine_similarity value: [tensor(0.0361), tensor(0.0323), tensor(0.0320), tensor(0.0320), tensor(0.0325)]
mean L1_Loss value: [tensor(0.1226), tensor(0.0738), tensor(0.0733), tensor(0.0732), tensor(0.0731)]
std L1_Loss value: [tensor(0.0122), tensor(0.0098), tensor(0.0098), tensor(0.0097), tensor(0.0098)]
mean cossim_gram_matrices value: [tensor(0.6797), tensor(0.9033), tensor(0.9045), tensor(0.9053), tensor(0.9044)]
std cossim_gram_matrices value: [tensor(0.0565), tensor(0.0418), tensor(0.0412), tensor(0.0412), tensor(0.0418)]
--------------------------------------------------------------------

from layer: layer2, to layer: G.blocks.2.0
time taken: 2.927586555480957
--------------------------------------------------------------------
--------------------------------------------------------------------
mean runtime: 2.891691255569458
std runtime: 0.07241951179952921




--------------------------------------------------------------------
from layer: layer2, to layer: G.blocks.3.0
time taken: 16.67423367500305
model str: resnet34
mean cosine_similarity value: [tensor(0.5609), tensor(0.8228)]
std cosine_similarity value: [tensor(0.0368), tensor(0.0300)]
mean L1_Loss value: [tensor(0.2627), tensor(0.1599)]
std L1_Loss value: [tensor(0.0241), tensor(0.0215)]
mean cossim_gram_matrices value: [tensor(0.8223), tensor(0.9579)]
std cossim_gram_matrices value: [tensor(0.0337), tensor(0.0211)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.3050), tensor(0.6092)]
std cosine_similarity value: [tensor(0.0426), tensor(0.0541)]
mean L1_Loss value: [tensor(0.0741), tensor(0.0531)]
std L1_Loss value: [tensor(0.0061), tensor(0.0063)]
mean cossim_gram_matrices value: [tensor(0.6842), tensor(0.9063)]
std cossim_gram_matrices value: [tensor(0.0574), tensor(0.0362)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4271), tensor(0.7782)]
std cosine_similarity value: [tensor(0.0342), tensor(0.0344)]
mean L1_Loss value: [tensor(0.1215), tensor(0.0723)]
std L1_Loss value: [tensor(0.0111), tensor(0.0096)]
mean cossim_gram_matrices value: [tensor(0.6448), tensor(0.8906)]
std cossim_gram_matrices value: [tensor(0.0559), tensor(0.0475)]
--------------------------------------------------------------------



--------------------------------------------------------------------
from layer: layer2, to layer: G.blocks.4.0
time taken: 16.54899573326111
model str: resnet34
mean cosine_similarity value: [tensor(0.5414), tensor(0.7671)]
std cosine_similarity value: [tensor(0.0274), tensor(0.0297)]
mean L1_Loss value: [tensor(0.2886), tensor(0.1853)]
std L1_Loss value: [tensor(0.0209), tensor(0.0210)]
mean cossim_gram_matrices value: [tensor(0.7891), tensor(0.9108)]
std cossim_gram_matrices value: [tensor(0.0267), tensor(0.0274)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.2832), tensor(0.5281)]
std cosine_similarity value: [tensor(0.0284), tensor(0.0448)]
mean L1_Loss value: [tensor(0.0833), tensor(0.0609)]
std L1_Loss value: [tensor(0.0050), tensor(0.0058)]
mean cossim_gram_matrices value: [tensor(0.6444), tensor(0.8072)]
std cossim_gram_matrices value: [tensor(0.0484), tensor(0.0521)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4203), tensor(0.7103)]
std cosine_similarity value: [tensor(0.0223), tensor(0.0344)]
mean L1_Loss value: [tensor(0.1316), tensor(0.0832)]
std L1_Loss value: [tensor(0.0095), tensor(0.0097)]
mean cossim_gram_matrices value: [tensor(0.6603), tensor(0.8291)]
std cossim_gram_matrices value: [tensor(0.0464), tensor(0.0538)]
--------------------------------------------------------------------


--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.1.0
time taken: 21.42864465713501
model str: resnet34
mean cosine_similarity value: [tensor(0.3404), tensor(0.3758), tensor(0.3774)]
std cosine_similarity value: [tensor(0.0389), tensor(0.0525), tensor(0.0532)]
mean L1_Loss value: [tensor(0.1528), tensor(0.1374), tensor(0.1365)]
std L1_Loss value: [tensor(0.0133), tensor(0.0147), tensor(0.0148)]
mean cossim_gram_matrices value: [tensor(0.5812), tensor(0.6229), tensor(0.6255)]
std cossim_gram_matrices value: [tensor(0.0562), tensor(0.0865), tensor(0.0870)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1601), tensor(0.2134), tensor(0.2150)]
std cosine_similarity value: [tensor(0.0327), tensor(0.0497), tensor(0.0505)]
mean L1_Loss value: [tensor(0.0307), tensor(0.0298), tensor(0.0297)]
std L1_Loss value: [tensor(0.0030), tensor(0.0028), tensor(0.0028)]
mean cossim_gram_matrices value: [tensor(0.5256), tensor(0.6147), tensor(0.6184)]
std cossim_gram_matrices value: [tensor(0.0787), tensor(0.1027), tensor(0.1044)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2493), tensor(0.3012), tensor(0.3031)]
std cosine_similarity value: [tensor(0.0263), tensor(0.0577), tensor(0.0580)]
mean L1_Loss value: [tensor(0.0611), tensor(0.0471), tensor(0.0469)]
std L1_Loss value: [tensor(0.0046), tensor(0.0058), tensor(0.0058)]
mean cossim_gram_matrices value: [tensor(0.3917), tensor(0.3950), tensor(0.3968)]
std cossim_gram_matrices value: [tensor(0.0518), tensor(0.1035), tensor(0.1040)]
--------------------------------------------------------------------


--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.2.0
time taken: 14.623576641082764
model str: resnet34
mean cosine_similarity value: [tensor(0.3549), tensor(0.6777)]
std cosine_similarity value: [tensor(0.0460), tensor(0.0435)]
mean L1_Loss value: [tensor(0.1442), tensor(0.0976)]
std L1_Loss value: [tensor(0.0138), tensor(0.0166)]
mean cossim_gram_matrices value: [tensor(0.5822), tensor(0.8642)]
std cossim_gram_matrices value: [tensor(0.0656), tensor(0.0361)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1836), tensor(0.4395)]
std cosine_similarity value: [tensor(0.0408), tensor(0.0528)]
mean L1_Loss value: [tensor(0.0298), tensor(0.0259)]
std L1_Loss value: [tensor(0.0027), tensor(0.0030)]
mean cossim_gram_matrices value: [tensor(0.5682), tensor(0.7896)]
std cossim_gram_matrices value: [tensor(0.0938), tensor(0.0694)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2632), tensor(0.6077)]
std cosine_similarity value: [tensor(0.0343), tensor(0.0506)]
mean L1_Loss value: [tensor(0.0581), tensor(0.0404)]
std L1_Loss value: [tensor(0.0048), tensor(0.0066)]
mean cossim_gram_matrices value: [tensor(0.3922), tensor(0.7759)]
std cossim_gram_matrices value: [tensor(0.0495), tensor(0.0543)]
--------------------------------------------------------------------

from layer: layer3, to layer: G.blocks.2.0
time taken: 2.674440860748291
--------------------------------------------------------------------
--------------------------------------------------------------------
mean runtime: 2.5831055641174316
std runtime: 0.06220612393238958




--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.3.0
time taken: 14.639167547225952
model str: resnet34
mean cosine_similarity value: [tensor(0.3360), tensor(0.5693)]
std cosine_similarity value: [tensor(0.0429), tensor(0.0552)]
mean L1_Loss value: [tensor(0.1423), tensor(0.1142)]
std L1_Loss value: [tensor(0.0126), tensor(0.0167)]
mean cossim_gram_matrices value: [tensor(0.5074), tensor(0.7630)]
std cossim_gram_matrices value: [tensor(0.0537), tensor(0.0628)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1753), tensor(0.3423)]
std cosine_similarity value: [tensor(0.0369), tensor(0.0526)]
mean L1_Loss value: [tensor(0.0283), tensor(0.0275)]
std L1_Loss value: [tensor(0.0026), tensor(0.0026)]
mean cossim_gram_matrices value: [tensor(0.5295), tensor(0.6898)]
std cossim_gram_matrices value: [tensor(0.0782), tensor(0.0907)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2508), tensor(0.4976)]
std cosine_similarity value: [tensor(0.0306), tensor(0.0582)]
mean L1_Loss value: [tensor(0.0609), tensor(0.0454)]
std L1_Loss value: [tensor(0.0049), tensor(0.0066)]
mean cossim_gram_matrices value: [tensor(0.3181), tensor(0.6390)]
std cossim_gram_matrices value: [tensor(0.0445), tensor(0.0753)]
--------------------------------------------------------------------


--------------------------------------------------------------------
from layer: layer3, to layer: G.blocks.4.0
time taken: 14.659619092941284
model str: resnet34
mean cosine_similarity value: [tensor(0.3069), tensor(0.3973)]
std cosine_similarity value: [tensor(0.0353), tensor(0.0573)]
mean L1_Loss value: [tensor(0.1509), tensor(0.1319)]
std L1_Loss value: [tensor(0.0123), tensor(0.0140)]
mean cossim_gram_matrices value: [tensor(0.3919), tensor(0.5817)]
std cossim_gram_matrices value: [tensor(0.0390), tensor(0.0850)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1467), tensor(0.2409)]
std cosine_similarity value: [tensor(0.0251), tensor(0.0508)]
mean L1_Loss value: [tensor(0.0298), tensor(0.0289)]
std L1_Loss value: [tensor(0.0027), tensor(0.0026)]
mean cossim_gram_matrices value: [tensor(0.3599), tensor(0.5851)]
std cossim_gram_matrices value: [tensor(0.0529), tensor(0.0929)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2370), tensor(0.3235)]
std cosine_similarity value: [tensor(0.0237), tensor(0.0609)]
mean L1_Loss value: [tensor(0.0659), tensor(0.0494)]
std L1_Loss value: [tensor(0.0041), tensor(0.0056)]
mean cossim_gram_matrices value: [tensor(0.2523), tensor(0.4316)]
std cossim_gram_matrices value: [tensor(0.0283), tensor(0.0975)]
--------------------------------------------------------------------








==> eval_values/imagenetval_500/gradient_descent.tex <==
no reg
---------------------------------------------------------------------------
regularization: none
layer1.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.9558640122413635
L1_Loss: 0.1592147946357727
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.665810763835907
L1_Loss: 0.0888051763176918
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.9872177839279175
L1_Loss: 0.018865186721086502
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 532.8814115524292
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 50/50 [14:32<00:00, 17.45s/it]
---------------------------------------------------------------------------
regularization: none
layer2.3.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.906747579574585
L1_Loss: 0.11364556849002838
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.6163038611412048
L1_Loss: 0.04893442988395691
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.9806650280952454
L1_Loss: 0.01503740344196558
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 872.0927364826202
---------------------------------------------------------------------------


---------------------------------------------------------------------------
regularization: none
layer3.5.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.6939141750335693
L1_Loss: 0.09596095234155655
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.39607566595077515
L1_Loss: 0.025504760444164276
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.950626015663147
L1_Loss: 0.010571456514298916
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 1285.593906402588
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 50/50 [26:27<00:00, 31.75s/it]
---------------------------------------------------------------------------
regularization: none
layer4.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.3571641743183136
L1_Loss: 1.084550380706787
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.13657762110233307
L1_Loss: 0.07984507828950882
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.9623086452484131
L1_Loss: 0.11399629712104797
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 1586.9843111038208
---------------------------------------------------------------------------



















with reg

---------------------------------------------------------------------------
regularization: jitter_only
layer1.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.9087986350059509
L1_Loss: 0.2404048591852188
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.6977603435516357
L1_Loss: 0.08482550084590912
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.9000964760780334
L1_Loss: 0.06955830752849579
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 596.8691837787628
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 50/50 [15:33<00:00, 18.66s/it]
---------------------------------------------------------------------------
regularization: jitter_only
layer2.3.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.8798105120658875
L1_Loss: 0.13359256088733673
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.6643995642662048
L1_Loss: 0.04692593961954117
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.8799855709075928
L1_Loss: 0.05244365334510803
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 932.7434895038605
---------------------------------------------------------------------------




---------------------------------------------------------------------------
regularization: jitter_only
layer3.5.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.7742980122566223
L1_Loss: 0.08114676922559738
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.5615028738975525
L1_Loss: 0.022849205881357193
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.8446049690246582
L1_Loss: 0.024336256086826324
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 1345.1021075248718
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 50/50 [27:22<00:00, 32.85s/it]
---------------------------------------------------------------------------
regularization: jitter_only
layer4.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity: 0.5517827272415161
L1_Loss: 0.9949548840522766
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity: 0.27580681443214417
L1_Loss: 0.09130147099494934
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity: 0.8647832274436951
L1_Loss: 0.22948050498962402
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 1642.0096783638
---------------------------------------------------------------------------

























no reg

0 [04:06<00:00, 24.68s/it]
---------------------------------------------------------------------------
regularization: none
layer1.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.9554126262664795
cosine_similarity standard deviation: 0.014232026413083076
L1_Loss mean: 0.15939006209373474
L1_Loss standard deviation: 0.034151412546634674
cossim_gram_matrices mean: 0.9884861707687378
cossim_gram_matrices standard deviation: 0.008256438188254833
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.7071136236190796
cosine_similarity standard deviation: 0.05634043738245964
L1_Loss mean: 0.07913035899400711
L1_Loss standard deviation: 0.010250085964798927
cossim_gram_matrices mean: 0.8001763820648193
cossim_gram_matrices standard deviation: 0.15114977955818176
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.9837898015975952
cosine_similarity standard deviation: 0.013109494000673294
L1_Loss mean: 0.021627046167850494
L1_Loss standard deviation: 0.009356859140098095
cossim_gram_matrices mean: 0.9897419214248657
cossim_gram_matrices standard deviation: 0.016298824921250343
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 245.6937
---------------------------------------------------------------------------



0 [06:26<00:00, 38.64s/it]
---------------------------------------------------------------------------
regularization: none
layer2.3.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.9087159633636475
cosine_similarity standard deviation: 0.01987684704363346
L1_Loss mean: 0.11179197579622269
L1_Loss standard deviation: 0.014560389332473278
cossim_gram_matrices mean: 0.9780054688453674
cossim_gram_matrices standard deviation: 0.013816540129482746
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.6464341878890991
cosine_similarity standard deviation: 0.03365449607372284
L1_Loss mean: 0.04828852042555809
L1_Loss standard deviation: 0.004074484575539827
cossim_gram_matrices mean: 0.8626518845558167
cossim_gram_matrices standard deviation: 0.07030563801527023
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.976425051689148
cosine_similarity standard deviation: 0.019166354089975357
L1_Loss mean: 0.017318913713097572
L1_Loss standard deviation: 0.006152957212179899
cossim_gram_matrices mean: 0.982556939125061
cossim_gram_matrices standard deviation: 0.02303370088338852
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 385.59938


layer3.5.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.7253679633140564
cosine_similarity standard deviation: 0.049786150455474854
L1_Loss mean: 0.08892428874969482
L1_Loss standard deviation: 0.014675094746053219
cossim_gram_matrices mean: 0.8464584946632385
cossim_gram_matrices standard deviation: 0.04501093178987503
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.46834269165992737
cosine_similarity standard deviation: 0.05025092884898186
L1_Loss mean: 0.025043360888957977
L1_Loss standard deviation: 0.002875208854675293
cossim_gram_matrices mean: 0.6960391998291016
cossim_gram_matrices standard deviation: 0.08981741219758987
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.9546931982040405
cosine_similarity standard deviation: 0.020038530230522156
L1_Loss mean: 0.010112007148563862
L1_Loss standard deviation: 0.0026271953247487545
cossim_gram_matrices mean: 0.9735515713691711
cossim_gram_matrices standard deviation: 0.020048845559358597
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 520.395



0 [09:39<00:00, 57.95s/it]
---------------------------------------------------------------------------
regularization: none
layer4.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.3690141439437866
cosine_similarity standard deviation: 0.06676068156957626
L1_Loss mean: 1.046199083328247
L1_Loss standard deviation: 0.10142353922128677
cossim_gram_matrices mean: 0.21501481533050537
cossim_gram_matrices standard deviation: 0.07573829591274261
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.16093595325946808
cosine_similarity standard deviation: 0.05733807384967804
L1_Loss mean: 0.08183116465806961
L1_Loss standard deviation: 0.022907324135303497
cossim_gram_matrices mean: 0.08324715495109558
cossim_gram_matrices standard deviation: 0.04874793067574501
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.9697385430335999
cosine_similarity standard deviation: 0.009108773432672024
L1_Loss mean: 0.10166696459054947
L1_Loss standard deviation: 0.020082276314496994
cossim_gram_matrices mean: 0.992222785949707
cossim_gram_matrices standard deviation: 0.003123265691101551
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 577.41738
---------------------------------------------------------------------------






jitter only

---------------------------------------------------------------------------
regularization: jitter_only
layer1.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.911055862903595
cosine_similarity standard deviation: 0.021204350516200066
L1_Loss mean: 0.23532088100910187
L1_Loss standard deviation: 0.043300312012434006
cossim_gram_matrices mean: 0.9782357215881348
cossim_gram_matrices standard deviation: 0.006035697180777788
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.7101979851722717
cosine_similarity standard deviation: 0.04627247154712677
L1_Loss mean: 0.08117136359214783
L1_Loss standard deviation: 0.013484111055731773
cossim_gram_matrices mean: 0.8972270488739014
cossim_gram_matrices standard deviation: 0.04481640085577965
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.9028438329696655
cosine_similarity standard deviation: 0.01736510545015335
L1_Loss mean: 0.06775126606225967
L1_Loss standard deviation: 0.010089006274938583
cossim_gram_matrices mean: 0.9513166546821594
cossim_gram_matrices standard deviation: 0.013185220770537853
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 261.36683440208435
---------------------------------------------------------------------------


---------------------------------------------------------------------------
regularization: jitter_only
layer2.3.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.882681667804718
cosine_similarity standard deviation: 0.015157985500991344
L1_Loss mean: 0.13121485710144043
L1_Loss standard deviation: 0.011607238091528416
cossim_gram_matrices mean: 0.9719573259353638
cossim_gram_matrices standard deviation: 0.011660217307507992
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.6754586696624756
cosine_similarity standard deviation: 0.03168458119034767
L1_Loss mean: 0.04626411199569702
L1_Loss standard deviation: 0.004093040246516466
cossim_gram_matrices mean: 0.9298180937767029
cossim_gram_matrices standard deviation: 0.033888500183820724
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.8841355443000793
cosine_similarity standard deviation: 0.02014557272195816
L1_Loss mean: 0.05099353939294815
L1_Loss standard deviation: 0.003854406299069524
cossim_gram_matrices mean: 0.9294642210006714
cossim_gram_matrices standard deviation: 0.028908073902130127
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 401.0168845653534
---------------------------------------------------------------------------

regularization: jitter_only
layer3.5.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.7820386290550232
cosine_similarity standard deviation: 0.041465874761343
L1_Loss mean: 0.07886142283678055
L1_Loss standard deviation: 0.013279324397444725
cossim_gram_matrices mean: 0.8939788341522217
cossim_gram_matrices standard deviation: 0.046568457037210464
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.5738667249679565
cosine_similarity standard deviation: 0.053083520382642746
L1_Loss mean: 0.022386563941836357
L1_Loss standard deviation: 0.002985636005178094
cossim_gram_matrices mean: 0.786567747592926
cossim_gram_matrices standard deviation: 0.09567739069461823
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.8534042835235596
cosine_similarity standard deviation: 0.027218956500291824
L1_Loss mean: 0.0232112854719162
L1_Loss standard deviation: 0.003664301009848714
cossim_gram_matrices mean: 0.9106773734092712
cossim_gram_matrices standard deviation: 0.028047999367117882
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 535.0939743518829


---------------------------------------------------------------------------
regularization: jitter_only
layer4.2.relu_2
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet34
cosine_similarity mean: 0.5700775384902954
cosine_similarity standard deviation: 0.09834124147891998
L1_Loss mean: 0.9782899618148804
L1_Loss standard deviation: 0.14623218774795532
cossim_gram_matrices mean: 0.5057933330535889
cossim_gram_matrices standard deviation: 0.13525232672691345
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: vgg19_bn
cosine_similarity mean: 0.29115691781044006
cosine_similarity standard deviation: 0.09011993557214737
L1_Loss mean: 0.09075219929218292
L1_Loss standard deviation: 0.023085754364728928
cossim_gram_matrices mean: 0.2782648801803589
cossim_gram_matrices standard deviation: 0.14373357594013214
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
model string: resnet50
cosine_similarity mean: 0.8692560195922852
cosine_similarity standard deviation: 0.03821203485131264
L1_Loss mean: 0.2240247279405594
L1_Loss standard deviation: 0.04260694980621338
cossim_gram_matrices mean: 0.9380027055740356
cossim_gram_matrices standard deviation: 0.029462547972798347
++++++++++++++++++++++++++++++++++++++++++++++++++++++++
time taken: 594.1219174861908
---------------------------------------------------------------------------







reconstruction times:
(no evaluation metrics)


---------------------------------------------------------------------------
regularization: none
layer1.2.relu_2
time taken: 237.56424689292908
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 10/10 [06:20<00:00, 38.08s/it]
---------------------------------------------------------------------------
regularization: none
layer2.3.relu_2
time taken: 379.8397727012634
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 10/10 [08:36<00:00, 51.63s/it]
---------------------------------------------------------------------------
regularization: none
layer3.5.relu_2
time taken: 515.4081437587738
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 10/10 [09:35<00:00, 57.58s/it]
---------------------------------------------------------------------------
regularization: none
layer4.2.relu_2
time taken: 574.8950667381287
---------------------------------------------------------------------------
done!



---------------------------------------------------------------------------
regularization: jitter_only
layer1.2.relu_2
time taken: 251.17594170570374
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 10/10 [06:35<00:00, 39.59s/it]
---------------------------------------------------------------------------
regularization: jitter_only
layer2.3.relu_2
time taken: 394.8146803379059
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 10/10 [08:51<00:00, 53.11s/it]
---------------------------------------------------------------------------
regularization: jitter_only
layer3.5.relu_2
time taken: 530.0824654102325
---------------------------------------------------------------------------
done!
create feature extractor...
create data loader...
load models...
100%|###########################################| 10/10 [09:50<00:00, 59.04s/it]
---------------------------------------------------------------------------
regularization: jitter_only
layer4.2.relu_2
time taken: 589.3796768188477
---------------------------------------------------------------------------
























==> eval_values/imagenetval_500/stylegan2.tex <==
trained on imagenet for one epoch



--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b64.conv0
time taken: 18.18737006187439
mean cossim value: [tensor(0.9151)]
std cossim value: [tensor(0.0245)]
mean cossim gram matrices value: [tensor(0.9889)]
std cossim gram matrices value: [tensor(0.0090)]
mean value l1: [tensor(0.2246)]
std value l1: [tensor(0.0462)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b128.conv0
time taken: 18.149105072021484
mean cossim value: [tensor(0.9306)]
std cossim value: [tensor(0.0215)]
mean cossim gram matrices value: [tensor(0.9907)]
std cossim gram matrices value: [tensor(0.0081)]
mean value l1: [tensor(0.2020)]
std value l1: [tensor(0.0424)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b256.conv0
time taken: 18.234293699264526
mean cossim value: [tensor(0.9254)]
std cossim value: [tensor(0.0214)]
mean cossim gram matrices value: [tensor(0.9901)]
std cossim gram matrices value: [tensor(0.0077)]
mean value l1: [tensor(0.2093)]
std value l1: [tensor(0.0418)]
--------------------------------------------------------------------



--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b32.conv0
time taken: 18.46910309791565
mean cossim value: [tensor(0.7926)]
std cossim value: [tensor(0.0306)]
mean cossim gram matrices value: [tensor(0.9558)]
std cossim gram matrices value: [tensor(0.0214)]
mean value l1: [tensor(0.1753)]
std value l1: [tensor(0.0215)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b64.conv0
time taken: 33.153987884521484
mean cossim value: [tensor(0.8476)]
std cossim value: [tensor(0.0242)]
mean cossim gram matrices value: [tensor(0.9710)]
std cossim gram matrices value: [tensor(0.0157)]
mean value l1: [tensor(0.1497)]
std value l1: [tensor(0.0181)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b128.conv0
time taken: 18.578863859176636
mean cossim value: [tensor(0.8481)]
std cossim value: [tensor(0.0232)]
mean cossim gram matrices value: [tensor(0.9723)]
std cossim gram matrices value: [tensor(0.0154)]
mean value l1: [tensor(0.1484)]
std value l1: [tensor(0.0170)]
--------------------------------------------------------------------





--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b16.conv0
time taken: 17.308685064315796
mean cossim value: [tensor(0.5269)]
std cossim value: [tensor(0.0699)]
mean cossim gram matrices value: [tensor(0.7543)]
std cossim gram matrices value: [tensor(0.0658)]
mean value l1: [tensor(0.1153)]
std value l1: [tensor(0.0205)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b32.conv0
time taken: 33.25621223449707
mean cossim value: [tensor(0.6337)]
std cossim value: [tensor(0.0481)]
mean cossim gram matrices value: [tensor(0.8210)]
std cossim gram matrices value: [tensor(0.0492)]
mean value l1: [tensor(0.1027)]
std value l1: [tensor(0.0183)]
--------------------------------------------------------------------
--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b64.conv0
time taken: 17.462701559066772
mean cossim value: [tensor(0.6706)]
std cossim value: [tensor(0.0432)]
mean cossim gram matrices value: [tensor(0.8447)]
std cossim gram matrices value: [tensor(0.0415)]
mean value l1: [tensor(0.0969)]
std value l1: [tensor(0.0169)]
--------------------------------------------------------------------





trained on afhq wild


--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b128.conv0
time taken: 14.647979259490967
model str: resnet34
mean cosine_similarity value: [tensor(0.9262)]
std cosine_similarity value: [tensor(0.0225)]
mean L1_Loss value: [tensor(0.2089)]
std L1_Loss value: [tensor(0.0430)]
mean cossim_gram_matrices value: [tensor(0.9884)]
std cossim_gram_matrices value: [tensor(0.0090)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.7677)]
std cosine_similarity value: [tensor(0.0585)]
mean L1_Loss value: [tensor(0.0695)]
std L1_Loss value: [tensor(0.0143)]
mean cossim_gram_matrices value: [tensor(0.9588)]
std cossim_gram_matrices value: [tensor(0.0289)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.9072)]
std cosine_similarity value: [tensor(0.0257)]
mean L1_Loss value: [tensor(0.0642)]
std L1_Loss value: [tensor(0.0114)]
mean cossim_gram_matrices value: [tensor(0.9667)]
std cossim_gram_matrices value: [tensor(0.0270)]
--------------------------------------------------------------------



--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b64.conv0
time taken: 32.170676708221436
mean cossim value: [tensor(0.8328)]
std cossim value: [tensor(0.0262)]
mean cossim gram matrices value: [tensor(0.9608)]
std cossim gram matrices value: [tensor(0.0211)]
mean value l1: [tensor(0.1572)]
std value l1: [tensor(0.0182)]
--------------------------------------------------------------------


--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b32.conv0
time taken: 32.831061124801636
mean cossim value: [tensor(0.5572)]
std cossim value: [tensor(0.0703)]
mean cossim gram matrices value: [tensor(0.7606)]
std cossim gram matrices value: [tensor(0.0733)]
mean value l1: [tensor(0.1161)]
std value l1: [tensor(0.0214)]
--------------------------------------------------------------------







trained on imagenet val



--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b16.conv0
time taken: 18.861555099487305
model str: resnet34
mean cosine_similarity value: [tensor(0.3420), tensor(0.5265)]
std cosine_similarity value: [tensor(0.0395), tensor(0.0707)]
mean L1_Loss value: [tensor(0.1453), tensor(0.1153)]
std L1_Loss value: [tensor(0.0141), tensor(0.0204)]
mean cossim_gram_matrices value: [tensor(0.5815), tensor(0.7535)]
std cossim_gram_matrices value: [tensor(0.0616), tensor(0.0674)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1828), tensor(0.3269)]
std cosine_similarity value: [tensor(0.0428), tensor(0.0587)]
mean L1_Loss value: [tensor(0.0319), tensor(0.0295)]
std L1_Loss value: [tensor(0.0033), tensor(0.0031)]
mean cossim_gram_matrices value: [tensor(0.5612), tensor(0.6835)]
std cossim_gram_matrices value: [tensor(0.0973), tensor(0.0908)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2640), tensor(0.4587)]
std cosine_similarity value: [tensor(0.0317), tensor(0.0766)]
mean L1_Loss value: [tensor(0.0566), tensor(0.0461)]
std L1_Loss value: [tensor(0.0055), tensor(0.0078)]
mean cossim_gram_matrices value: [tensor(0.4082), tensor(0.6404)]
std cossim_gram_matrices value: [tensor(0.0598), tensor(0.0899)]
--------------------------------------------------------------------















--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b64.conv0
time taken: 28.384428024291992
model str: resnet34
mean cosine_similarity value: [tensor(0.7274), tensor(0.9146)]
std cosine_similarity value: [tensor(0.0353), tensor(0.0247)]
mean L1_Loss value: [tensor(0.4283), tensor(0.2254)]
std L1_Loss value: [tensor(0.0510), tensor(0.0465)]
mean cossim_gram_matrices value: [tensor(0.9234), tensor(0.9887)]
std cossim_gram_matrices value: [tensor(0.0333), tensor(0.0087)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.4823), tensor(0.7419)]
std cosine_similarity value: [tensor(0.0578), tensor(0.0667)]
mean L1_Loss value: [tensor(0.1128), tensor(0.0738)]
std L1_Loss value: [tensor(0.0143), tensor(0.0159)]
mean cossim_gram_matrices value: [tensor(0.7881), tensor(0.9558)]
std cossim_gram_matrices value: [tensor(0.0935), tensor(0.0323)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.6542), tensor(0.8952)]
std cosine_similarity value: [tensor(0.0436), tensor(0.0283)]
mean L1_Loss value: [tensor(0.1368), tensor(0.0683)]
std L1_Loss value: [tensor(0.0149), tensor(0.0121)]
mean cossim_gram_matrices value: [tensor(0.8145), tensor(0.9687)]
std cossim_gram_matrices value: [tensor(0.0717), tensor(0.0255)]
--------------------------------------------------------------------

--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b128.conv0
time taken: 27.850098848342896
model str: resnet34
mean cosine_similarity value: [tensor(0.7265), tensor(0.9303)]
std cosine_similarity value: [tensor(0.0285), tensor(0.0216)]
mean L1_Loss value: [tensor(0.4362), tensor(0.2023)]
std L1_Loss value: [tensor(0.0436), tensor(0.0426)]
mean cossim_gram_matrices value: [tensor(0.9203), tensor(0.9905)]
std cossim_gram_matrices value: [tensor(0.0287), tensor(0.0079)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.4321), tensor(0.7753)]
std cosine_similarity value: [tensor(0.0453), tensor(0.0592)]
mean L1_Loss value: [tensor(0.1212), tensor(0.0684)]
std L1_Loss value: [tensor(0.0118), tensor(0.0147)]
mean cossim_gram_matrices value: [tensor(0.7844), tensor(0.9643)]
std cossim_gram_matrices value: [tensor(0.1017), tensor(0.0277)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.6407), tensor(0.9142)]
std cosine_similarity value: [tensor(0.0352), tensor(0.0239)]
mean L1_Loss value: [tensor(0.1375), tensor(0.0612)]
std L1_Loss value: [tensor(0.0132), tensor(0.0109)]
mean cossim_gram_matrices value: [tensor(0.8122), tensor(0.9734)]
std cossim_gram_matrices value: [tensor(0.0646), tensor(0.0230)]
--------------------------------------------------------------------

--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b256.conv0
time taken: 25.230903387069702
model str: resnet34
mean cosine_similarity value: [tensor(0.7175), tensor(0.9252)]
std cosine_similarity value: [tensor(0.0290), tensor(0.0220)]
mean L1_Loss value: [tensor(0.4531), tensor(0.2096)]
std L1_Loss value: [tensor(0.0417), tensor(0.0426)]
mean cossim_gram_matrices value: [tensor(0.8952), tensor(0.9898)]
std cossim_gram_matrices value: [tensor(0.0428), tensor(0.0087)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.4468), tensor(0.7745)]
std cosine_similarity value: [tensor(0.0586), tensor(0.0562)]
mean L1_Loss value: [tensor(0.1152), tensor(0.0683)]
std L1_Loss value: [tensor(0.0107), tensor(0.0142)]
mean cossim_gram_matrices value: [tensor(0.6837), tensor(0.9683)]
std cossim_gram_matrices value: [tensor(0.1542), tensor(0.0275)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.6239), tensor(0.9070)]
std cosine_similarity value: [tensor(0.0387), tensor(0.0243)]
mean L1_Loss value: [tensor(0.1448), tensor(0.0638)]
std L1_Loss value: [tensor(0.0143), tensor(0.0109)]
mean cossim_gram_matrices value: [tensor(0.7526), tensor(0.9766)]
std cossim_gram_matrices value: [tensor(0.0935), tensor(0.0215)]
--------------------------------------------------------------------






--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b32.conv0
time taken: 21.67950940132141
model str: resnet34
mean cosine_similarity value: [tensor(0.5284), tensor(0.7913)]
std cosine_similarity value: [tensor(0.0316), tensor(0.0311)]
mean L1_Loss value: [tensor(0.2836), tensor(0.1759)]
std L1_Loss value: [tensor(0.0225), tensor(0.0219)]
mean cossim_gram_matrices value: [tensor(0.8406), tensor(0.9548)]
std cossim_gram_matrices value: [tensor(0.0442), tensor(0.0212)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.2775), tensor(0.5780)]
std cosine_similarity value: [tensor(0.0277), tensor(0.0501)]
mean L1_Loss value: [tensor(0.0780), tensor(0.0567)]
std L1_Loss value: [tensor(0.0057), tensor(0.0064)]
mean cossim_gram_matrices value: [tensor(0.7518), tensor(0.9111)]
std cossim_gram_matrices value: [tensor(0.0729), tensor(0.0415)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4257), tensor(0.7440)]
std cosine_similarity value: [tensor(0.0318), tensor(0.0349)]
mean L1_Loss value: [tensor(0.1295), tensor(0.0802)]
std L1_Loss value: [tensor(0.0110), tensor(0.0103)]
mean cossim_gram_matrices value: [tensor(0.7319), tensor(0.8975)]
std cossim_gram_matrices value: [tensor(0.0722), tensor(0.0474)]
--------------------------------------------------------------------



--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b64.conv0
time taken: 65.88876628875732
model str: resnet34
mean cosine_similarity value: [tensor(0.5525), tensor(0.8467), tensor(0.8463), tensor(0.8471), tensor(0.8462), tensor(0.8468), tensor(0.8466)]
std cosine_similarity value: [tensor(0.0341), tensor(0.0265), tensor(0.0259), tensor(0.0253), tensor(0.0262), tensor(0.0262), tensor(0.0262)]
mean L1_Loss value: [tensor(0.2717), tensor(0.1493), tensor(0.1492), tensor(0.1490), tensor(0.1494), tensor(0.1493), tensor(0.1494)]
std L1_Loss value: [tensor(0.0237), tensor(0.0190), tensor(0.0185), tensor(0.0186), tensor(0.0186), tensor(0.0186), tensor(0.0188)]
mean cossim_gram_matrices value: [tensor(0.8452), tensor(0.9710), tensor(0.9718), tensor(0.9732), tensor(0.9718), tensor(0.9723), tensor(0.9723)]
std cossim_gram_matrices value: [tensor(0.0426), tensor(0.0165), tensor(0.0161), tensor(0.0147), tensor(0.0158), tensor(0.0156), tensor(0.0154)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.2918), tensor(0.6659), tensor(0.6643), tensor(0.6645), tensor(0.6637), tensor(0.6649), tensor(0.6639)]
std cosine_similarity value: [tensor(0.0332), tensor(0.0465), tensor(0.0464), tensor(0.0468), tensor(0.0469), tensor(0.0471), tensor(0.0469)]
mean L1_Loss value: [tensor(0.0753), tensor(0.0499), tensor(0.0497), tensor(0.0498), tensor(0.0499), tensor(0.0499), tensor(0.0499)]
std L1_Loss value: [tensor(0.0062), tensor(0.0057), tensor(0.0056), tensor(0.0057), tensor(0.0056), tensor(0.0056), tensor(0.0057)]
mean cossim_gram_matrices value: [tensor(0.7476), tensor(0.9399), tensor(0.9400), tensor(0.9421), tensor(0.9390), tensor(0.9411), tensor(0.9415)]
std cossim_gram_matrices value: [tensor(0.0751), tensor(0.0321), tensor(0.0324), tensor(0.0314), tensor(0.0310), tensor(0.0307), tensor(0.0314)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4469), tensor(0.8175), tensor(0.8175), tensor(0.8190), tensor(0.8178), tensor(0.8179), tensor(0.8178)]
std cosine_similarity value: [tensor(0.0340), tensor(0.0296), tensor(0.0289), tensor(0.0272), tensor(0.0286), tensor(0.0289), tensor(0.0293)]
mean L1_Loss value: [tensor(0.1254), tensor(0.0668), tensor(0.0667), tensor(0.0665), tensor(0.0667), tensor(0.0667), tensor(0.0667)]
std L1_Loss value: [tensor(0.0111), tensor(0.0086), tensor(0.0084), tensor(0.0082), tensor(0.0083), tensor(0.0083), tensor(0.0085)]
mean cossim_gram_matrices value: [tensor(0.7246), tensor(0.9361), tensor(0.9370), tensor(0.9410), tensor(0.9374), tensor(0.9384), tensor(0.9388)]
std cossim_gram_matrices value: [tensor(0.0717), tensor(0.0370), tensor(0.0374), tensor(0.0336), tensor(0.0344), tensor(0.0353), tensor(0.0354)]
--------------------------------------------------------------------




--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b128.conv0
time taken: 18.891572952270508
model str: resnet34
mean cosine_similarity value: [tensor(0.5742), tensor(0.8473)]
std cosine_similarity value: [tensor(0.0350), tensor(0.0239)]
mean L1_Loss value: [tensor(0.2593), tensor(0.1489)]
std L1_Loss value: [tensor(0.0236), tensor(0.0174)]
mean cossim_gram_matrices value: [tensor(0.8555), tensor(0.9717)]
std cossim_gram_matrices value: [tensor(0.0370), tensor(0.0150)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.3176), tensor(0.6635)]
std cosine_similarity value: [tensor(0.0360), tensor(0.0417)]
mean L1_Loss value: [tensor(0.0727), tensor(0.0495)]
std L1_Loss value: [tensor(0.0062), tensor(0.0053)]
mean cossim_gram_matrices value: [tensor(0.7691), tensor(0.9385)]
std cossim_gram_matrices value: [tensor(0.0667), tensor(0.0306)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4661), tensor(0.8205)]
std cosine_similarity value: [tensor(0.0351), tensor(0.0268)]
mean L1_Loss value: [tensor(0.1186), tensor(0.0662)]
std L1_Loss value: [tensor(0.0111), tensor(0.0079)]
mean cossim_gram_matrices value: [tensor(0.7368), tensor(0.9388)]
std cossim_gram_matrices value: [tensor(0.0673), tensor(0.0341)]
--------------------------------------------------------------------














--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b32.conv0
time taken: 63.04427480697632
model str: resnet34
mean cosine_similarity value: [tensor(0.3384), tensor(0.6344), tensor(0.6387), tensor(0.6392), tensor(0.6400), tensor(0.6414), tensor(0.6393)]
std cosine_similarity value: [tensor(0.0366), tensor(0.0494), tensor(0.0505), tensor(0.0494), tensor(0.0496), tensor(0.0485), tensor(0.0492)]
mean L1_Loss value: [tensor(0.1466), tensor(0.1020), tensor(0.1014), tensor(0.1014), tensor(0.1014), tensor(0.1012), tensor(0.1014)]
std L1_Loss value: [tensor(0.0137), tensor(0.0182), tensor(0.0183), tensor(0.0183), tensor(0.0184), tensor(0.0180), tensor(0.0182)]
mean cossim_gram_matrices value: [tensor(0.5551), tensor(0.8262), tensor(0.8287), tensor(0.8297), tensor(0.8288), tensor(0.8303), tensor(0.8285)]
std cossim_gram_matrices value: [tensor(0.0508), tensor(0.0471), tensor(0.0471), tensor(0.0451), tensor(0.0456), tensor(0.0452), tensor(0.0458)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1665), tensor(0.4206), tensor(0.4234), tensor(0.4225), tensor(0.4249), tensor(0.4247), tensor(0.4235)]
std cosine_similarity value: [tensor(0.0364), tensor(0.0501), tensor(0.0506), tensor(0.0501), tensor(0.0502), tensor(0.0492), tensor(0.0493)]
mean L1_Loss value: [tensor(0.0303), tensor(0.0271), tensor(0.0271), tensor(0.0271), tensor(0.0270), tensor(0.0270), tensor(0.0271)]
std L1_Loss value: [tensor(0.0032), tensor(0.0031), tensor(0.0031), tensor(0.0030), tensor(0.0031), tensor(0.0030), tensor(0.0031)]
mean cossim_gram_matrices value: [tensor(0.5130), tensor(0.7406), tensor(0.7457), tensor(0.7458), tensor(0.7465), tensor(0.7470), tensor(0.7466)]
std cossim_gram_matrices value: [tensor(0.0933), tensor(0.0855), tensor(0.0865), tensor(0.0850), tensor(0.0844), tensor(0.0851), tensor(0.0837)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2668), tensor(0.5758), tensor(0.5808), tensor(0.5809), tensor(0.5822), tensor(0.5828), tensor(0.5814)]
std cosine_similarity value: [tensor(0.0279), tensor(0.0550), tensor(0.0549), tensor(0.0542), tensor(0.0546), tensor(0.0542), tensor(0.0547)]
mean L1_Loss value: [tensor(0.0584), tensor(0.0414), tensor(0.0412), tensor(0.0412), tensor(0.0411), tensor(0.0411), tensor(0.0412)]
std L1_Loss value: [tensor(0.0051), tensor(0.0071), tensor(0.0071), tensor(0.0071), tensor(0.0071), tensor(0.0070), tensor(0.0071)]
mean cossim_gram_matrices value: [tensor(0.3947), tensor(0.7439), tensor(0.7495), tensor(0.7518), tensor(0.7504), tensor(0.7530), tensor(0.7512)]
std cossim_gram_matrices value: [tensor(0.0510), tensor(0.0691), tensor(0.0685), tensor(0.0668), tensor(0.0669), tensor(0.0664), tensor(0.0672)]
--------------------------------------------------------------------


--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b64.conv0
time taken: 18.6317138671875
model str: resnet34
mean cosine_similarity value: [tensor(0.3528), tensor(0.6693)]
std cosine_similarity value: [tensor(0.0396), tensor(0.0437)]
mean L1_Loss value: [tensor(0.1429), tensor(0.0972)]
std L1_Loss value: [tensor(0.0137), tensor(0.0168)]
mean cossim_gram_matrices value: [tensor(0.5585), tensor(0.8430)]
std cossim_gram_matrices value: [tensor(0.0512), tensor(0.0427)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.1767), tensor(0.4490)]
std cosine_similarity value: [tensor(0.0364), tensor(0.0467)]
mean L1_Loss value: [tensor(0.0293), tensor(0.0261)]
std L1_Loss value: [tensor(0.0030), tensor(0.0029)]
mean cossim_gram_matrices value: [tensor(0.5167), tensor(0.7618)]
std cossim_gram_matrices value: [tensor(0.0835), tensor(0.0799)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.2701), tensor(0.6117)]
std cosine_similarity value: [tensor(0.0291), tensor(0.0495)]
mean L1_Loss value: [tensor(0.0604), tensor(0.0394)]
std L1_Loss value: [tensor(0.0048), tensor(0.0065)]
mean cossim_gram_matrices value: [tensor(0.3977), tensor(0.7639)]
std cossim_gram_matrices value: [tensor(0.0500), tensor(0.0661)]
--------------------------------------------------------------------







trained on afhq



--------------------------------------------------------------------
from layer: layer1, to layer: G.synthesis.b128.conv0
time taken: 14.333183288574219
model str: resnet34
mean cosine_similarity value: [tensor(0.9262)]
std cosine_similarity value: [tensor(0.0225)]
mean L1_Loss value: [tensor(0.2089)]
std L1_Loss value: [tensor(0.0430)]
mean cossim_gram_matrices value: [tensor(0.9884)]
std cossim_gram_matrices value: [tensor(0.0090)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.7677)]
std cosine_similarity value: [tensor(0.0585)]
mean L1_Loss value: [tensor(0.0695)]
std L1_Loss value: [tensor(0.0143)]
mean cossim_gram_matrices value: [tensor(0.9588)]
std cossim_gram_matrices value: [tensor(0.0289)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.9072)]
std cosine_similarity value: [tensor(0.0257)]
mean L1_Loss value: [tensor(0.0642)]
std L1_Loss value: [tensor(0.0114)]
mean cossim_gram_matrices value: [tensor(0.9667)]
std cossim_gram_matrices value: [tensor(0.0270)]
--------------------------------------------------------------------

from layer: layer1, to layer: G.synthesis.b128.conv0
time taken: 5.785789966583252
--------------------------------------------------------------------
--------------------------------------------------------------------
mean runtime: 5.875071692466736
std runtime: 0.1756018960162651






--------------------------------------------------------------------
from layer: layer2, to layer: G.synthesis.b64.conv0
time taken: 10.77894115447998
model str: resnet34
mean cosine_similarity value: [tensor(0.8335)]
std cosine_similarity value: [tensor(0.0277)]
mean L1_Loss value: [tensor(0.1562)]
std L1_Loss value: [tensor(0.0191)]
mean cossim_gram_matrices value: [tensor(0.9621)]
std cossim_gram_matrices value: [tensor(0.0202)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.6447)]
std cosine_similarity value: [tensor(0.0430)]
mean L1_Loss value: [tensor(0.0512)]
std L1_Loss value: [tensor(0.0053)]
mean cossim_gram_matrices value: [tensor(0.9234)]
std cossim_gram_matrices value: [tensor(0.0370)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.7990)]
std cosine_similarity value: [tensor(0.0321)]
mean L1_Loss value: [tensor(0.0704)]
std L1_Loss value: [tensor(0.0089)]
mean cossim_gram_matrices value: [tensor(0.9165)]
std cossim_gram_matrices value: [tensor(0.0429)]
--------------------------------------------------------------------

from layer: layer2, to layer: G.synthesis.b64.conv0
time taken: 5.62726354598999
--------------------------------------------------------------------
--------------------------------------------------------------------
mean runtime: 5.721486735343933
std runtime: 0.0897825696579809





--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b32.conv0
time taken: 9.645459413528442
model str: resnet34
mean cosine_similarity value: [tensor(0.5623)]
std cosine_similarity value: [tensor(0.0695)]
mean L1_Loss value: [tensor(0.1144)]
std L1_Loss value: [tensor(0.0215)]
mean cossim_gram_matrices value: [tensor(0.7713)]
std cossim_gram_matrices value: [tensor(0.0678)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.3609)]
std cosine_similarity value: [tensor(0.0613)]
mean L1_Loss value: [tensor(0.0286)]
std L1_Loss value: [tensor(0.0033)]
mean cossim_gram_matrices value: [tensor(0.6994)]
std cossim_gram_matrices value: [tensor(0.0969)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.4963)]
std cosine_similarity value: [tensor(0.0746)]
mean L1_Loss value: [tensor(0.0462)]
std L1_Loss value: [tensor(0.0083)]
mean cossim_gram_matrices value: [tensor(0.6622)]
std cossim_gram_matrices value: [tensor(0.0883)]
--------------------------------------------------------------------


from layer: layer3, to layer: G.synthesis.b32.conv0
time taken: 5.85716700553894
--------------------------------------------------------------------
--------------------------------------------------------------------
mean runtime: 5.601062679290772
std runtime: 0.1409771795226982





--------------------------------------------------------------------
from layer: layer3, to layer: G.synthesis.b64.conv0
time taken: 8.759999752044678
model str: resnet34
mean cosine_similarity value: [tensor(0.5831)]
std cosine_similarity value: [tensor(0.0617)]
mean L1_Loss value: [tensor(0.1123)]
std L1_Loss value: [tensor(0.0201)]
mean cossim_gram_matrices value: [tensor(0.7746)]
std cossim_gram_matrices value: [tensor(0.0636)]
--------------------------------------------------------------------
model str: vgg19_bn
mean cosine_similarity value: [tensor(0.3741)]
std cosine_similarity value: [tensor(0.0561)]
mean L1_Loss value: [tensor(0.0281)]
std L1_Loss value: [tensor(0.0031)]
mean cossim_gram_matrices value: [tensor(0.6993)]
std cossim_gram_matrices value: [tensor(0.0904)]
--------------------------------------------------------------------
model str: resnet50
mean cosine_similarity value: [tensor(0.5181)]
std cosine_similarity value: [tensor(0.0687)]
mean L1_Loss value: [tensor(0.0456)]
std L1_Loss value: [tensor(0.0079)]
mean cossim_gram_matrices value: [tensor(0.6703)]
std cossim_gram_matrices value: [tensor(0.0869)]
--------------------------------------------------------------------








==> eval_values/misc/plot_values.tex <==
import numpy as np
import matplotlib.pyplot as plt
import torch



plt.rcParams.update({'font.size': 22})



x = ["Layer1", "Layer2", "Layer3", "Layer4"]
x_ = ["Layer1", "Layer2", "Layer3"]
stylegan2 = [0.954, 0.878, 0.778, 0.527]
stylegan2_error = [0.008, 0.015, 0.032, 0.117]

biggan = [0.930, 0.835, ]
biggan_error = [0.008, 0.015, 0.032]


gd_no_reg = [0.973, 0.928, 0.729, 0.319]
gd_no_reg_error = [0.006, 0.010, 0.040, 0.024]


gd_with_reg = [0.932, 0.903, 0.831, 0.665]
gd_with_reg_error = [0.010, 0.009, 0.024, 0.053]



plt.figure(figsize=(15, 10))
#plt.plot(x, stylegan2, '--bo', markersize=22)
plt.errorbar(x, stylegan2, stylegan2_error, fmt='--bo', markersize=10)
plt.errorbar(x, gd_no_reg, gd_no_reg_error, fmt='--rx', markersize=10)
plt.errorbar(x, gd_with_reg, gd_with_reg_error, fmt='--gp', markersize=10)

plt.legend((["StyleGAN2", "no reg", "with reg"]),
            shadow=True)
plt.xlabel("Layer")
plt.ylabel("Cosine Similarity")
plt.show()


























